Sparse Tensor Transpositions

We present a new algorithm for transposing sparse tensors called Quesadilla. The algorithm converts the sparse tensor data structure to a list of coordinates and sorts it with a fast multi-pass radix algorithm that exploits knowledge of the requested transposition and the tensors input partial coordinate ordering to provably minimize the number of parallel partial sorting passes. We evaluate both a serial and a parallel implementation of Quesadilla on a set of 19 tensors from the FROSTT collection, a set of tensors taken from scientific and data analytic applications. We compare Quesadilla and a generalization, Top-2-sadilla to several state of the art approaches, including the tensor transposition routine used in the SPLATT tensor factorization library. In serial tests, Quesadilla was the best strategy for 60% of all tensor and transposition combinations and improved over SPLATT by at least 19% in half of the combinations. In parallel tests, at least one of Quesadilla or Top-2-sadilla was the best strategy for 52% of all tensor and transposition combinations.

==> Makefile <==
pdf: main.pdf
.PHONY: pdf

main.pdf: 
	latexmk -pdf main.tex
.PHONY: main.pdf

notodo:
	latexmk -pdf -pdflatex='pdflatex %O -interaction=nonstopmode -synctex=1 "\def\notodo{1}\input{%S}"'main.tex
.PHONY: notodo

main.ps: main.pdf
	acroread -toPostScript $<

clean:
	latexmk -C main.tex
	rm -f *.bbl *.log
.PHONY: clean

view: main.pdf
	open main.pdf
.PHONY: view

skim: main.pdf
	open -a "Skim" main.pdf
.PHONY: skim

safe: main.pdf
	mkdir -p archive
	cp $^ archive/`date "+%y.%m.%d-%H.%M.%S"`-`openssl md5 < $^`.pdf

SPELLTEX := $(shell ./bin/get-tex-files.sh main.tex)
spell:
	@ for i in $(SPELLTEX); do aspell --mode=tex -p ./aspell.words -c $$i; done
	@ for i in $(SPELLTEX); do perl bin/double.pl $$i; done
	@ for i in $(SPELLTEX); do perl bin/abbrv.pl  $$i; done
	@ bash bin/hyphens.sh $(SPELLTEX)
	@ ( head -1 aspell.words ; tail -n +2 aspell.words | sort ) > aspell.words~
	@ mv aspell.words~ aspell.words
.PHONY: spell


